Dissecting Medical Referral Mechanisms in Health Services: Role of Physician Professional Networks

Medical referrals between primary care physicians (PC) and specialist care (SC) physicians profoundly impact patient care regarding quality, satisfaction, and cost. This paper investigates the influence of professional networks among medical doctors on referring patients from PC to SC. Using five-year consultation data from a Portuguese private health provider, we conducted exploratory data analysis and constructed both professional and referral networks among physicians. We then apply Graph Neural Network (GNN) models to learn latent representations of the referral network. Our analysis supports the hypothesis that doctors' professional social connections can predict medical referrals, potentially enhancing collaboration within organizations and improving healthcare services. This research contributes to dissecting the underlying mechanisms in primary-specialty referrals, thereby providing valuable insights for enhancing patient care and effective healthcare management.

==> 00_plos_to_submit_main.tex <==
\input{preamble}

\begin{document}

\input{01_title_page}

\input{02_abstract}

\linenumbers

\input{03_body}

\input{04_Supporting_Information}


%\section*{Acknowledgments}
%This work was partially supported by the strategic project NOVA LINCS (UIDB/04516/2020), and FCT, IP project CMU/TIC/0016/2021, The authors would like to thank CUF Health for sharing the data.



\nolinenumbers

\bibliography{bibliography} 

\end{document}


==> 01_title_page.tex <==

%% As in https://journals.plos.org/plosone/s/file?id=3fac/PLOS%20Affiliations%20Formatting%20Guidelines.pdf

\vspace*{0.2in}

% Title must be 250 characters or less.
\begin{flushleft}
{\Large
\textbf\newline{Dissecting Medical Referral Mechanisms in Health Service using Graph Neural Networks} % Please use "sentence case" for title and headings (capitalize only the first word in a title (or heading), the first word in a subtitle (or subheading), and any proper nouns).
}
\newline
% Insert author names, affiliations and corresponding author email (do not include titles, positions, or degrees).
\\
Regina de Brito Duarte\textsuperscript{1*}, %2\Yinyang},
Qiwei Han\textsuperscript{2\ddag}, %\Yinyang},
Claudia Soares\textsuperscript{3\ddag}% \textcurrency},

%%%%%%%%%%%%%%%%%%%% IMCOMPLETE%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\bigskip
\textbf{1} Instituto Superior Tecnico, Lisbon, Portugal
\\
\textbf{2} Data Science Knowledge Center, Nova School of Business and Economics, Lisbon, Portugal
\\
\textbf{3} NOVA LINCS, Computer Science Department, NOVA School of Science and Technology, Universidade NOVA de Lisboa, Caparica, Portugal.
\\
\bigskip

% Insert additional author notes using the symbols described below. Insert symbol callouts after author names as necessary.
% 
% Remove or comment out the author notes below if they aren't used.
%
% Primary Equal Contribution Note
%\Yinyang These authors contributed equally to this work.

% Additional Equal Contribution Note
% Also use this double-dagger symbol for special authorship notes, such as senior authorship.
%\ddag These authors also contributed equally to this work.
\ddag These authors contributed equally to this work.

% Current address notes
%\textcurrency Current Address: Dept/Program/Center, Institution Name, City, State, Country % change symbol to "\textcurrency a" if more than one current address note
% \textcurrency b Insert second current address 
% \textcurrency c Insert third current address

% Deceased author note
%\dag Deceased

% Group/Consortium Author Note
%\textpilcrow Membership list can be found in the Acknowledgments section.

% Use the asterisk to denote corresponding authorship and provide email address in note below.
* reginaduarte@tecnico.ulisboa.pt



\end{flushleft}



==> 02_abstract.tex <==
\section*{Abstract}
Medical referrals between primary care doctors and specialists affect many aspects of patient care, such as quality of care, patient satisfaction, and health care costs. 


In this work, we hypothesize that the social network of medical doctors can influence the referral process. We analyze primary-specialty referrals through transaction data over medical appointments gathered between 2012 and 2017 in all hospital centers of an European private health provider. The main objective of the study is to discover patterns and hidden mechanisms in primary-specialty referrals to improve the efficiency of health care services. First, we carry out exploratory data analysis and search for patterns or interesting features of the data and afterwords, we create and analyze the doctor's social network and the referrals network. We learn the representation of the referral network using a Graph Neural Network (GNN). Finally, we discuss the node's representation of the referral network, which supports our main hypothesis that the social connections of the doctors are predictive of the medical referrals. 
This work addresses the discovery of important patterns in medical referrals to, in future work, improve the efficiency of collaboration within organizations.




